Reproducing Adaptive Reranking for Reasoning-Intensive IR

The classical cascading pipeline of retrieve--rerank suffers from a bounded recall problem, stemming from limitations of the first-stage retriever. Most current approaches address the bounded recall problem by improving the first-stage retriever, but this incurs substantial training and inference costs, especially to handle queries that require substantial reasoning. To circumvent the computational costs of reasoning-based retrievers, we replicate the findings of GAR, Graph-based Adaptive Reranking, on the BRIGHT reasoning-intensive retrieval benchmark. GAR addresses the bounded recall problem by modifying the reranking process itself through iterative exploration of a corpus graph, but it was previously only tested on models designed for topical and question-answering-style queries. Hence, reproduce GAR in reasoning-intensive settings with reasoning and non-reasoning reranking models. We observe that the quality of the reranker's signal plays an important role in identifying additional relevant documents within the corpus graph. Overall, we find that GAR boosts the effectiveness of reasoning-intensive retrieval across a variety of models while contributing minimally to computational overheads. Ultimately, this work enables more practical deployment of retrieval systems that can address reasoning-intensive queries.

==> method.tex <==
\section{A Recap of \gar{}}
\label{sec:method}
\gar{} solves \textit{bounded-recall} problem by adaptively reranking documents. For a given reranking budget $c$, it starts with selecting $b$ documents from the initially retrieved documents list (denoted by $R_{0}$). Then, a pointwise reranker (a cross encoder such as MonoT5) is applied to rerank these $b$ documents, and then these documents are added to the final rank list (denoted as $R_1$). Then, a graph frontier ($F$) is prepared using the neighbors of already reranked documents. For this, the \textit{offline} built corpus graph is looked up. In the graph frontier, each neighbor is assigned the score of the source document given by the ranker. By this, the neighbors of highly reranked documents are prioritized based on the \textit{clustering hypothesis}, and therefore the feedback from the reranker (quantified by relevance score) becomes crucial. 
For the next batch, the top $b$ documents from the graph frontier $F$ are selected and ranked. Next, these documents are added to the final rank list $R_1$. Then, the graph frontier $F$ is updated with the neighbors of these newly ranked documents. \gar{} keeps selecting batches from $R_0$ and graph frontier $F$ alternatively until the reranking criteria is met, i.e, $|R_1|=c$. 


==> rel_work.tex <==
\section{Related Work}
\label{sec:rel_work}


Recent advancements in document ranking have increasingly relied on complex rankers based on transformer models and, more recently, instruction-tuned models. They are highly effective in providing precise relevance estimates, but computationally expensive. 
We contextualize our work into hybrid retrieval, adaptive retrieval, and other related ideas on online adaptation for rankings.


\subsection{Hybrid Retrieval and Telescoping}

Retrieval functions such as BM25 are generally designed to provide fast but less precise relevance estimates. In contrast, complex rankers, including cross-encoders and LLMs, offer far more accurate relevance assessments at the expense of significant computational resources. 
Due to this tradeoff, complex rankers are typically applied as final-stage ranking functions in a telescoping framework (also referred to as \textit{cascading} or \textit{multi-stage} ranking) \cite{matveeva2006high}. 
In this framework, an initial ranking is conducted using computationally inexpensive methods like BM25, and only a subset of top-ranked documents is passed to the final stage, where more expensive machine-learned models calculate the final ranking scores.
Consequently telescoping paradigm is widely adopted across a variety of domains where strict latency requirements are paramount: web search, e-commerce and live fact-checking systems.
Note that there is no restriction on what can be used as a retriever in the first stage. 
Historically lexical retrieval or BM25~\cite{bm25,splade, wang2011cascade} was mostly used as a retrieval function. 
In more modern search systems dense retrieval~\cite{lin2021batch, karpukhin-etal-2020-dense}, learned sparse~\cite{DBLP:conf/sigir/MacAvaneyN0TGF20b,splade}, and hybrid sparse-dense ensembles are used for first-stage retrieval~\cite{ cormack2009reciprocal,bruch2023analysis, chen2022out,wang2021bert}. 

However, telescoping suffers from a key limitation when the retrieval scores from the first stage do not accurately reflect the relevance of the documents. Retrieval scores are typically used to first-rank documents, and the top-k documents are selected for re-ranking based on their retrieval scores. Since this selection process is typically conducted in a single step, any failure to capture relevant documents in the top-k results can lead to poor recall, ultimately degrading precision in the final rankings. Furthermore, documents that are not passed to the re-ranking stage remain ranked solely according to their initial retrieval scores, which may not reflect their true relevance.

To improve the quality by improving recall, either higher retrieval depths are considered~\cite{leonhardt2022efficient,bruch2023analysis}, hybrid retrieval~\cite{bruch2023analysis,cormack2009reciprocal,hybrid-rank-lu2022zero} or query expansions techniques are employed~\cite{carpineto2012survey}.
However, the choice of documents to rank is still dependent on the retriever score.
Unlike these approaches, we dynamically update the relevance estimates for all retrieved candidates by iteratively ranking smaller batches of documents, resulting in improved recall. 
\vspace{-1.2em}
\subsection{Adaptive Retrieval}
The closest approaches to ours are the recently proposed Adaptive Retrieval (AR) methods introduced by~\citet{macavaney2022adaptive}. These methods operate on a corpus graph (constructed during an offline phase), which encodes document-document similarities based on lexical or semantic features.
Adaptive retrieval methods alternate between the initially retrieved results and the corpus graph neighborhoods of re-ranked documents to select a batch for re-ranking. These methods are fundamentally based on the Clustering Hypothesis~\cite{jardine1971use}, which assumes that relevant documents tend to cluster together in the feature space. In \gar{}~\cite{macavaney2022adaptive}, only the neighbors of previously ranked documents are explored. More recently, \textsc{Quam}~\cite{rathee2024quam} improved upon \gar{} by selecting documents based on their degree of relatedness to the re-ranked documents.

In contrast to \gar{} and \textsc{Quam}, which rely on cross-encoders for ranking, \citet{kulkarni2023lexically} proposed a method that uses bi-encoders to re-rank documents. Their approach selects only seed documents from the initial retrieved results and continues exploring the corpus graph neighborhood until the re-ranking budget is exhausted.
While adaptive retrieval methods dynamically schedule documents to the ranker, their alternating strategy is heuristic-driven and sample-inefficient. In contrast, our online relevance estimation framework generalizes and simplifies the adaptive retrieval paradigm, offering significant improvements in sample efficiency.

Partially related to our approach are ideas from online learning to rank~\cite{zoghi2017online,grotov2016online,li2019onlineltrs}, which learn the parameters of ranking models from user interaction data. However, our approach differs fundamentally from this line of work. Unlike these methods, we do not rely on direct user feedback or address challenges like prioritizing or de-biasing rank-sensitive clicks. Moreover, our framework operates on a significantly smaller feature space, allowing it to scale efficiently to large retrieval sizes compared to learning-to-rank models. Other similar works include~\citet{reddy2023inference} and \citet{DBLP:journals/corr/abs-2306-09657}, which learn a new query representation online during re-ranking. Unlike these methods, we use a bandit-based framework and continually refine query representations, thereby selecting better candidate documents at each inference step.

